Accelerating LLM Reasoning via Early Rejection with Partial Reward Modeling

Large Language Models (LLMs) are increasingly relied upon for solving complex reasoning tasks in domains such as mathematics, logic, and multi-step question answering. A growing line of work seeks to improve reasoning quality by scaling inference time compute particularly through Process Reward Models (PRMs), used to reward the reasoning at intermediate steps. While effective, these methods introduce substantial computational overhead, especially when generating large numbers of solutions in parallel. In this paper, we investigate whether PRMs can be used mid-generation to provide early signals that enable the rejection of suboptimal candidates before full generation of step is complete. We introduce the hypothesis that PRMs are also Partial Reward Models, meaning that the scores they assign to partially completed reasoning step are predictive of final output quality. This allows for principled early rejection based on intermediate token-level signals. We support this hypothesis both theoretically, by proving that the risk of discarding optimal beams decreases exponentially with generation length and empirically, by demonstrating a strong correlation between partial and final rewards across multiple reward models. On math reasoning benchmarks, our method achieves up to 1.4$\times$-9$\times$ reduction in inference FLOPs without degrading final performance. These results suggest that early rejection is a powerful mechanism for improving the compute-efficiency of reasoning in LLMs.

==> Figures/table_1.tex <==
\definecolor{dpink}{HTML}{EAD5DC}
\definecolor{pink}{HTML}{EEE3E7}
\definecolor{lightgreen}{HTML}{E8F0E6}
\definecolor{lightred}{HTML}{F4E8E6}

\begin{table}[t]
% \resizebox{1\textwidth}{!}
\scriptsize
{%
\begin{tabular}{c|c|ccccc}
\noalign{\hrule height 1pt} 
\rowcolor{dpink}
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\end{tabular}}} & \multicolumn{5}{c}{\textit{\textbf{Number of Beams (N)}}} \\ 

\cline{3-7} 
\rowcolor{dpink}
 \textbf{\textit{PRM}}&\textbf{\textit{Method}}& \multicolumn{1}{c|}{\textbf{4}} & \multicolumn{1}{c|}{\textbf{8}} & \multicolumn{1}{c|}{\textbf{16}} & \multicolumn{1}{c|}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} \\
 
\hline
\rowcolor{pink}
\multicolumn{7}{c}{\textit{\textbf{Llama-3.2-3B}}}
\cline{2-8}

\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{MM7B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} & 37.14 & 38.76 & 39.55 & 40.38 & 43.12 \\
& & 1.32 & 7.48 & 15.47 & 31.21 & 80.34 \\
\cline{2-7}  
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  & &  & \\
& & & & &  &  \\
\cline{2-7} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  32.57 & 35.82 & 38.81 & 40.36 & \\
& & 0.24 & 1.08 & 4.34 & 14.85 & \\

\cline{1-7}

\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{S1.5B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} & &  & &  & \\
& & & & &  &  \\
\cline{2-7}  
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  & &  & \\
& & & & &  &  \\
\cline{2-7} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} & & &  & &   \\
& & & & &  &  \\

\cline{1-7}
\hline
\rowcolor{pink}
\multicolumn{7}{c}{\textit{\textbf{Qwen2.5-3B}}}
\cline{2-8}

\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{MM7B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} & &  & &  & \\
& & & & &  &  \\
\cline{2-7}  
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  & &  & \\
& & & & &  &  \\
\cline{2-7} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  &  & &  & \\
& & & & &  &  \\

\cline{1-7}

\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{S1.5B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} & &  & &  & \\
& & & & &  &  \\
\cline{2-7}  
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  & &  & \\
& & & & &  &  \\
\cline{2-7} 
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  &  & &  & \\
& & & & &  &  \\

\hline
\hline
\noalign{\hrule height 1pt}

\end{tabular}
}
\caption{Accuracy (percent) and total FLOPs ($\times 10^{18}$) for beams 4 to 64 for different LLM, PRM and early rejection configurations. We compare standard PRM-guided beam search (Vanilla) with our approach using partial reward thresholds at $\tau = 32$ and $\tau = 64$. 
% Early rejection consistently reduces compute cost without sacrificing performance, with stronger gains at larger $N$.
Abbreviations: \textbf{MM7B} (MathShepherd-Mistral-7B), \textbf{S1.5B} (Skywork-PRM-1.5B)}
\label{table:main_small}
\end{table}

==> Figures/table_2.tex <==
\begin{table}[t]
% \resizebox{1\textwidth}{!}
\scriptsize
{%
\begin{tabular}{c|c|c|ccccc}
\noalign{\hrule height 1pt} 
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LLM\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}PRM\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Method\end{tabular}}} & \multicolumn{5}{c}{\textit{\textbf{Number of Beams (N)}}} \\ 

\cline{4-8} 
 & & & \multicolumn{1}{c|}{\textbf{4}} & \multicolumn{1}{c|}{\textbf{8}} & \multicolumn{1}{c|}{\textbf{16}} & \multicolumn{1}{c|}{\textbf{32}} & \multicolumn{1}{c}{\textbf{64}} \\
\hline
\hline

\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{}\end{tabular}} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{MM7B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} & 37.14 & 38.76 & 39.55 & 40.38 & 43.12 \\
& & & 1.32 & 7.48 & 15.47 & 31.21 & 80.34 \\
\cline{3-8}  
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\
\cline{3-8} 
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\

\cline{2-8}

& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{S1.5B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} &  &  &  &  & \\
& & & & &  &  & \\
\cline{3-8}  
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\
\cline{3-8}
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\

\hline
\hline

\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{Q3B}\end{tabular}} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{MM7B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} &  &  &  &  & \\
& & & & &  &  & \\
\cline{3-8}  
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\
\cline{3-8} 
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\

\cline{2-8}

& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}
\textbf{S1.5B}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Vanilla\end{tabular}} &  &  &  &  & \\
& & & & &  &  & \\
\cline{3-8}  
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=32\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\
\cline{3-8}
& & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
$\tau$=64\end{tabular}} &  &  &  &  &  \\
& & & & &  &  &  \\

\hline
\hline
\noalign{\hrule height 1pt}

\end{tabular}
}
\caption{Accuracy (percent) and total FLOPs ($\times 10^{18}$) for beams 4 to 64 for different LLM, PRM and early rejection configurations. We compare standard PRM-guided beam search (Vanilla) with our approach using partial reward thresholds at $\tau = 32$ and $\tau = 64$. 
% Early rejection consistently reduces compute cost without sacrificing performance, with stronger gains at larger $N$.
Abbreviations: \textbf{L3B} (Llama-3.2-3B), \textbf{Q3B} (Qwen2.5-3B), \textbf{MM7B} (MathShepherd-Mistral-7B), \textbf{S1.5B} (Skywork-PRM-1.5B)}
\label{table:main_small}
\end{table}


==> macros.tex <==
\usepackage{natbib} 

\usepackage{xspace}
\newcommand{\proj}{LADs\xspace}

\newcommand{\ali}[1]{\noindent\textcolor{red}{\bf Ali: #1}}
\newcommand{\azal}[1]{\noindent\textcolor{purple}{\bf Azal: #1}}
\usepackage{booktabs} % Ensure this is included for \toprule, \midrule, etc

\newcommand{\taskitem}[2]{%
  \vspace{3pt}
  \begin{tikzpicture}
%    [baseline=(X.base)]\node [drop shadow,fill=white,draw,thin,text width=0.94\textwidth] (X) {{\em #1} {\bf #2}};
\node[draw=none,shade,
%      top color=blue!30,   
%      bottom color=blue!2,
      top color=taskbgcol,
      bottom color=taskbgcol!25,
      rounded corners=6pt,
      text width=0.94\textwidth,
      blur shadow={shadow blur steps=5},
      shadow xshift=0.7em,
      shadow yshift=-0.7em,
    ] {{\em #1} {\bf #2}};
  \end{tikzpicture}
  \vspace{5pt}
}

\usepackage[most]{tcolorbox}
\usepackage{subcaption}

\usepackage{pifont}
